Multimodal Lecture Presentations Dataset: Understanding Multimodality in Educational Slides

Lecture slide presentations, a sequence of pages that contain text and figures accompanied by speech, are constructed and presented carefully in order to optimally transfer knowledge to students. Previous studies in multimedia and psychology attribute the effectiveness of lecture presentations to their multimodal nature. As a step toward developing AI to aid in student learning as intelligent teacher assistants, we introduce the Multimodal Lecture Presentations dataset as a large-scale benchmark testing the capabilities of machine learning models in multimodal understanding of educational content. Our dataset contains aligned slides and spoken language, for 180+ hours of video and 9000+ slides, with 10 lecturers from various subjects (e.g., computer science, dentistry, biology). We introduce two research tasks which are designed as stepping stones towards AI agents that can explain (automatically captioning a lecture presentation) and illustrate (synthesizing visual figures to accompany spoken explanations) educational content. We provide manual annotations to help implement these two research tasks and evaluate state-of-the-art models on them. Comparing baselines and human student performances, we find that current models struggle in (1) weak crossmodal alignment between slides and spoken text, (2) learning novel visual mediums, (3) technical language, and (4) long-range sequences. Towards addressing this issue, we also introduce PolyViLT, a multimodal transformer trained with a multi-instance learning loss that is more effective than current approaches. We conclude by shedding light on the challenges and opportunities in multimodal understanding of educational presentations.

==> y82_metadata.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[H]
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}l|l@{}}
\toprule
Title & Multimodal Lecture Presentations (MLP) Dataset \\ \midrule
Description & A dataset to develop AI models capable of understanding multimodal information present in lecture slides \\ \midrule
Keyword & multimodal learning, crossmodal retrieval, education, vision and language, intelligent tutoring systems \\ \midrule
modified & 06/15/22 \\ \midrule
publisher & MultiComp Lab, Carnegie Mellon University \\ \midrule
contactPoint & Dong Won Lee, datasetmlp@gmail.com \\ \midrule
{\color[HTML]{000000} accessLevel} & public \\ \midrule
license & CC BY-NC-SA 4.0 \\ \bottomrule
\end{tabular}%
\caption{Metadata of MLP Dataset}
\label{tab:metadata}
}
\end{table}

==> z87_figure_k.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcccccc@{}}
 & \multicolumn{3}{c}{Fig2Text} & \multicolumn{3}{c}{Text2Fig} \\
K = & bio-1 & dental & ml-1 & {\color[HTML]{1E1E1E} bio-1} & {\color[HTML]{1E1E1E} dental} & {\color[HTML]{1E1E1E} ml-1} \\
1 & 26.18 ± 3.92 & 12.15 ± 1.67 & 12.58 ± 4.62 & 28.74 ± 1.32 & {\color[HTML]{1E1E1E} 12.32 ± 1.37} & {\color[HTML]{1E1E1E} 22.23 ± 3.83} \\
3 & 24.26 ± 11.1 & 14.06 ± 4.52 & 13.12 ± 1.37 & 26.74 ± 2.94 & {\color[HTML]{1E1E1E} 14.79 ± 6.27} & {\color[HTML]{1E1E1E} 19.84 ± 1.66} \\
5 & \textbf{33.35 ± 3.27} & 9.53 ± 0.72 & 13.47 ± 3.73 & \textbf{35.91 ± 3.27} & {\color[HTML]{1E1E1E} 14.82 ± 0.72} & {\color[HTML]{1E1E1E} 21.81 ± 3.73} \\
7 & 31.29 ± 7.51 & \textbf{17.07 ± 1.66} & 19.32 ± 3.04 & {\color[HTML]{1E1E1E} 32.24 ± 5.25} & {\color[HTML]{1E1E1E} \textbf{20.23 ± 0.12}} & {\color[HTML]{1E1E1E} \textbf{24.84 ± 8.93}} \\
9 & 33.5 ± 4.64 & 15.18 ± 3.58 & \textbf{22.24 ± 1.62} & {\color[HTML]{1E1E1E} 31.06 ± 7.43} & {\color[HTML]{1E1E1E} 16.08 ± 5.18} & {\color[HTML]{1E1E1E} 19.2 ± 4.04}
\end{tabular}%
}
\end{table}

==> z96_continual.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|lll|lll|lll}
\hline
Speaker & \multicolumn{3}{l|}{psy-1} & \multicolumn{3}{l|}{ml-1} & \multicolumn{3}{l}{bio-1} \\ \hline
Method & ACC & FWT & BWT & ACC & FWT & BWT & ACC & FWT & BWT \\ \hline
Fine-Tune & 0.213 & -0.14 & -0.223 &  &  &  &  &  &  \\
EWC &  &  &  &  &  &  &  &  &  \\
GEM &  &  &  &  &  &  &  &  &  \\
Others? &  &  &  &  &  &  &  &  &  \\ \hline
\end{tabular}%
}
\caption{Continual Learning Metrics for Crossmodal Retrieval }
\end{table}

==> z97_dataset.tex <==
\begin{figure}[h]
\includegraphics[width=0.99\linewidth]{figs/dataset.png}
\caption{Example of a slide in the dataset}
\end{figure}



==> z98_sample_span.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% \begin{table}[]
% \begin{tabular}{@{}lll@{}}
% \toprule
% Query & mollusca can includes a hundred thousand species and again they are based on having these different parts of their body the first one is the {[}MASK{]} and that's really how we separate these groups out and so you may hear it instead of a nudibranch you may hear it as a gastropod which means stomach foot that's like the stale or the snails and the Slugs where they ride on the {[}BLANK{]} and so that's why they call it the stomach foot you have the bivalves which are the clams and the oysters in that stuff &  \\ \midrule
% Passage & \textbf{phylum mollusca the lophotrochozoan phylum mollusca includes 100,000 species the body of a mollusc has three main parts that vary in size and form: a muscular foot,  usually used for movement a visceral mass containing most of the internal organs a mantle a fold of tissue that drapes over the visceral mass and secretes a shell if present} &  \\
% Answer & muscular foot &  \\ \bottomrule
% \end{tabular}
% \end{table}
\begin{table}[]
\begin{tabularx}{\textwidth}{l|X}
%   \textbf{Symptom} & \textbf{Metric} \\
% \hline
 Spoken Language: \\ Query & mollusca can includes a hundred thousand species and again they are based on having these different parts of their body the first one is the {[}MASK{]} and that's really how we separate these groups out and so you may hear it instead of a nudibranch you may hear it as a gastropod which means stomach foot that's like the stale or the snails and the Slugs where they ride on the {[}MASK{]} and so that's why they call it the stomach foot you have the bivalves which are the clams and the oysters in that stuff\\
\hline
Slide Text: \\ Passage  & phylum mollusca the lophotrochozoan phylum mollusca includes 100,000 species the body of a mollusc has three main parts that vary in size and form: a muscular foot,  usually used for movement a visceral mass containing most of the internal organs a mantle a fold of tissue that drapes over the visceral mass and secretes a shell if present\\
\hline
Answer & muscular foot\\

\end{tabularx}
\vspace{2mm}
\caption{Example of a Span Selection Task}
\label{span_ex}
\end{table}

==> z99_CMR_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}l|llllllllll|l@{}}
\toprule
Model & anat-1 & bio-3 & dental & ml-1 & psy-1 & psy-2 & speaking & bio-1 & anat-2 & bio-4 & Average \\ \midrule
PVSE & \textbf{12.11} & \textbf{9.12} & \textbf{5.23} & 9.01 & 39.37 & \textbf{45.54} & 14.50 & 6.28 & \textbf{17.87} & 12.99 & 17.20 \\
PCME & 8.70 & 9.37 & \textbf{4.51} & \textbf{10.40} & \textbf{43.09} & 43.36 & \textbf{14.62} & \textbf{6.55} & 17.49 & \textbf{14.55} & \textbf{17.26} \\
CLIP & 7.24 & 5.88 & 3.02 & 6.39 & 23.74 & 26.78 & 7.67 & 4.255 & 9.42 & 12.77 & 10.71 \\ \bottomrule
\end{tabular}%
}
\vspace{2mm}
\caption{Sum of Recall@10 Scores for Image-to-Text and Text-to-Image}
\end{table}
